Calpha: Toward Native Biomolecular Intelligence in a General-Purpose Language Model

Biomolecular foundation models predict the structures of proteins and their complexes accurately, and large language models (LLMs) reason in natural language, but the two remain separate: the abilities of the former are not part of a general-purpose LLM, and the reasoning of the latter does not enter a structure prediction. Calpha aims at one general model that folds proteins and complexes, understands protein sequence and structure, and lets its language reasoning influence the structures it predicts. This report covers the first step, in which an LLM outputs single-chain protein structures. Qwen3.5-9B reads a sequence enriched with ESM2 residue features. It can respond in text or emit a token that invokes a pretrained SimpleFold structure head, which receives information about the protein only through Qwen's residue states. Under a fixed folding request, the head achieves mean TM-scores of 0.808 on the FoldBench-334 development set, 0.635 on CASP16 domains and 0.900 on a CAMEO-style PDB set. We compare these predictions with a baseline in which ESM2-3B encodes the sequence and a fine-tuned SimpleFold-3B head predicts the coordinates. The two systems also differ in trainable weights, training duration and crop length. For chains of 100--299 residues, all three paired confidence intervals include zero. At 300--600 residues, the mean differences are -0.044, -0.160 and -0.025, respectively. In a separate test, four English request types triggered folding on every evaluated example. Protein training reduced accuracy on a 350-item MMLU-Pro subset from 77.4% to 70.3%. An LLM can therefore output single-chain structures from its own states, with lower long-chain scores in the current comparisons and reduced accuracy on the evaluated MMLU-Pro subset. Complex prediction, structure understanding and the effect of language reasoning on the predicted coordinates remain future work.

==> numbers.tex <==
% Tables and macros use the numerical snapshot in numbers.json. See README.md.
\makeatletter
\newcommand{\N}[1]{\@ifundefined{N@#1}{\textcolor{red}{[pending]}}{\@nameuse{N@#1}}}
\@namedef{N@biomatrix_1p7b.cameo2025.family}{0.259}
\@namedef{N@biomatrix_1p7b.cameo2025.len100-300}{0.292}
\@namedef{N@biomatrix_1p7b.cameo2025.len300-600}{0.214}
\@namedef{N@biomatrix_1p7b.cameo2025.len<100}{0.205}
\@namedef{N@biomatrix_1p7b.cameo2025.len>600}{0.138}
\@namedef{N@biomatrix_1p7b.cameo2025.no_family}{0.169}
\@namedef{N@biomatrix_1p7b.cameo2025.overall}{0.252}
\@namedef{N@biomatrix_1p7b.cameo2025.subset}{0.236}
\@namedef{N@biomatrix_1p7b.casp16.family}{0.166}
\@namedef{N@biomatrix_1p7b.casp16.len100-300}{0.175}
\@namedef{N@biomatrix_1p7b.casp16.len300-600}{0.138}
\@namedef{N@biomatrix_1p7b.casp16.len<100}{0.230}
\@namedef{N@biomatrix_1p7b.casp16.len>600}{0.073}
\@namedef{N@biomatrix_1p7b.casp16.no_family}{0.172}
\@namedef{N@biomatrix_1p7b.casp16.overall}{0.169}
\@namedef{N@biomatrix_1p7b.casp16.subset}{0.183}
\@namedef{N@biomatrix_1p7b.foldbench334.family}{0.159}
\@namedef{N@biomatrix_1p7b.foldbench334.len100-300}{0.168}
\@namedef{N@biomatrix_1p7b.foldbench334.len300-600}{0.146}
\@namedef{N@biomatrix_1p7b.foldbench334.len<100}{0.195}
\@namedef{N@biomatrix_1p7b.foldbench334.len>600}{0.119}
\@namedef{N@biomatrix_1p7b.foldbench334.no_family}{0.170}
\@namedef{N@biomatrix_1p7b.foldbench334.overall}{0.163}
\@namedef{N@biomatrix_1p7b.foldbench334.subset}{0.184}
\@namedef{N@biomatrix_4b.cameo2025.family}{0.326}
\@namedef{N@biomatrix_4b.cameo2025.len100-300}{0.363}
\@namedef{N@biomatrix_4b.cameo2025.len300-600}{0.270}
\@namedef{N@biomatrix_4b.cameo2025.len<100}{0.205}
\@namedef{N@biomatrix_4b.cameo2025.len>600}{0.099}
\@namedef{N@biomatrix_4b.cameo2025.no_family}{0.145}
\@namedef{N@biomatrix_4b.cameo2025.overall}{0.311}
\@namedef{N@biomatrix_4b.cameo2025.subset}{0.247}
\@namedef{N@biomatrix_4b.casp16.family}{0.166}
\@namedef{N@biomatrix_4b.casp16.len100-300}{0.171}
\@namedef{N@biomatrix_4b.casp16.len300-600}{0.119}
\@namedef{N@biomatrix_4b.casp16.len<100}{0.242}
\@namedef{N@biomatrix_4b.casp16.len>600}{0.064}
\@namedef{N@biomatrix_4b.casp16.no_family}{0.161}
\@namedef{N@biomatrix_4b.casp16.overall}{0.163}
\@namedef{N@biomatrix_4b.casp16.subset}{0.174}
\@namedef{N@biomatrix_4b.foldbench334.family}{0.155}
\@namedef{N@biomatrix_4b.foldbench334.len100-300}{0.168}
\@namedef{N@biomatrix_4b.foldbench334.len300-600}{0.135}
\@namedef{N@biomatrix_4b.foldbench334.len<100}{0.187}
\@namedef{N@biomatrix_4b.foldbench334.len>600}{0.101}
\@namedef{N@biomatrix_4b.foldbench334.no_family}{0.164}
\@namedef{N@biomatrix_4b.foldbench334.overall}{0.158}
\@namedef{N@biomatrix_4b.foldbench334.subset}{0.176}
\@namedef{N@dplm2_650m.cameo2025.family}{0.770}
\@namedef{N@dplm2_650m.cameo2025.len100-300}{0.806}
\@namedef{N@dplm2_650m.cameo2025.len300-600}{0.722}
\@namedef{N@dplm2_650m.cameo2025.len<100}{0.668}
\@namedef{N@dplm2_650m.cameo2025.len>600}{0.445}
\@namedef{N@dplm2_650m.cameo2025.no_family}{0.608}
\@namedef{N@dplm2_650m.cameo2025.overall}{0.757}
\@namedef{N@dplm2_650m.cameo2025.subset}{0.762}
\@namedef{N@dplm2_650m.casp16.family}{0.586}
\@namedef{N@dplm2_650m.casp16.len100-300}{0.545}
\@namedef{N@dplm2_650m.casp16.len300-600}{0.435}
\@namedef{N@dplm2_650m.casp16.len<100}{0.561}
\@namedef{N@dplm2_650m.casp16.len>600}{0.303}
\@namedef{N@dplm2_650m.casp16.no_family}{0.428}
\@namedef{N@dplm2_650m.casp16.overall}{0.515}
\@namedef{N@dplm2_650m.casp16.subset}{0.543}
\@namedef{N@dplm2_650m.foldbench334.family}{0.702}
\@namedef{N@dplm2_650m.foldbench334.len100-300}{0.635}
\@namedef{N@dplm2_650m.foldbench334.len300-600}{0.731}
\@namedef{N@dplm2_650m.foldbench334.len<100}{0.621}
\@namedef{N@dplm2_650m.foldbench334.len>600}{0.510}
\@namedef{N@dplm2_650m.foldbench334.no_family}{0.582}
\@namedef{N@dplm2_650m.foldbench334.overall}{0.656}
\@namedef{N@dplm2_650m.foldbench334.subset}{0.619}
\@namedef{N@dplm2p1.cameo2025.family}{0.852}
\@namedef{N@dplm2p1.cameo2025.len100-300}{0.848}
\@namedef{N@dplm2p1.cameo2025.len300-600}{0.823}
\@namedef{N@dplm2p1.cameo2025.len<100}{0.758}
\@namedef{N@dplm2p1.cameo2025.len>600}{0.551}
\@namedef{N@dplm2p1.cameo2025.no_family}{0.557}
\@namedef{N@dplm2p1.cameo2025.overall}{0.828}
\@namedef{N@dplm2p1.cameo2025.subset}{0.814}
\@namedef{N@dplm2p1.casp16.family}{0.614}
\@namedef{N@dplm2p1.casp16.len100-300}{0.547}
\@namedef{N@dplm2p1.casp16.len300-600}{0.516}
\@namedef{N@dplm2p1.casp16.len<100}{0.481}
\@namedef{N@dplm2p1.casp16.len>600}{0.359}
\@namedef{N@dplm2p1.casp16.no_family}{0.421}
\@namedef{N@dplm2p1.casp16.overall}{0.527}
\@namedef{N@dplm2p1.casp16.subset}{0.529}
\@namedef{N@dplm2p1.foldbench334.family}{0.745}
\@namedef{N@dplm2p1.foldbench334.len100-300}{0.653}
\@namedef{N@dplm2p1.foldbench334.len300-600}{0.760}
\@namedef{N@dplm2p1.foldbench334.len<100}{0.598}
\@namedef{N@dplm2p1.foldbench334.len>600}{0.616}
\@namedef{N@dplm2p1.foldbench334.no_family}{0.564}
\@namedef{N@dplm2p1.foldbench334.overall}{0.676}
\@namedef{N@dplm2p1.foldbench334.subset}{0.640}
\@namedef{N@esm2_direct.cameo2025.family}{0.928}
\@namedef{N@esm2_direct.cameo2025.len100-300}{0.929}
\@namedef{N@esm2_direct.cameo2025.len300-600}{0.921}
\@namedef{N@esm2_direct.cameo2025.len<100}{0.828}
\@namedef{N@esm2_direct.cameo2025.len>600}{0.666}
\@namedef{N@esm2_direct.cameo2025.no_family}{0.791}
\@namedef{N@esm2_direct.cameo2025.overall}{0.917}
\@namedef{N@esm2_direct.cameo2025.subset}{0.915}
\@namedef{N@esm2_direct.casp16.family}{0.758}
\@namedef{N@esm2_direct.casp16.len100-300}{0.696}
\@namedef{N@esm2_direct.casp16.len300-600}{0.702}
\@namedef{N@esm2_direct.casp16.len<100}{0.610}
\@namedef{N@esm2_direct.casp16.len>600}{0.489}
\@namedef{N@esm2_direct.casp16.no_family}{0.589}
\@namedef{N@esm2_direct.casp16.overall}{0.682}
\@namedef{N@esm2_direct.casp16.subset}{0.682}
\@namedef{N@esm2_direct.foldbench334.family}{0.850}
\@namedef{N@esm2_direct.foldbench334.len100-300}{0.813}
\@namedef{N@esm2_direct.foldbench334.len300-600}{0.861}
\@namedef{N@esm2_direct.foldbench334.len<100}{0.833}
\@namedef{N@esm2_direct.foldbench334.len>600}{0.598}
\@namedef{N@esm2_direct.foldbench334.no_family}{0.776}
\@namedef{N@esm2_direct.foldbench334.overall}{0.822}
\@namedef{N@esm2_direct.foldbench334.subset}{0.818}
\@namedef{N@esm3_open.cameo2025.family}{0.862}
\@namedef{N@esm3_open.cameo2025.len100-300}{0.870}
\@namedef{N@esm3_open.cameo2025.len300-600}{0.850}
\@namedef{N@esm3_open.cameo2025.len<100}{0.783}
\@namedef{N@esm3_open.cameo2025.len>600}{0.568}
\@namedef{N@esm3_open.cameo2025.no_family}{0.739}
\@namedef{N@esm3_open.cameo2025.overall}{0.852}
\@namedef{N@esm3_open.cameo2025.subset}{0.844}
\@namedef{N@esm3_open.casp16.family}{0.725}
\@namedef{N@esm3_open.casp16.len100-300}{0.664}
\@namedef{N@esm3_open.casp16.len300-600}{0.619}
\@namedef{N@esm3_open.casp16.len<100}{0.599}
\@namedef{N@esm3_open.casp16.len>600}{0.527}
\@namedef{N@esm3_open.casp16.no_family}{0.543}
\@namedef{N@esm3_open.casp16.overall}{0.643}
\@namedef{N@esm3_open.casp16.subset}{0.659}
\@namedef{N@esm3_open.foldbench334.family}{0.829}
\@namedef{N@esm3_open.foldbench334.len100-300}{0.757}
\@namedef{N@esm3_open.foldbench334.len300-600}{0.875}
\@namedef{N@esm3_open.foldbench334.len<100}{0.708}
\@namedef{N@esm3_open.foldbench334.len>600}{0.805}
\@namedef{N@esm3_open.foldbench334.no_family}{0.720}
\@namedef{N@esm3_open.foldbench334.overall}{0.787}
\@namedef{N@esm3_open.foldbench334.subset}{0.760}
\@namedef{N@esmfold.cameo2025.family}{0.910}
\@namedef{N@esmfold.cameo2025.len100-300}{0.911}
\@namedef{N@esmfold.cameo2025.len300-600}{0.912}
\@namedef{N@esmfold.cameo2025.len<100}{0.839}
\@namedef{N@esmfold.cameo2025.len>600}{0.737}
\@namedef{N@esmfold.cameo2025.no_family}{0.855}
\@namedef{N@esmfold.cameo2025.overall}{0.905}
\@namedef{N@esmfold.cameo2025.subset}{0.902}
\@namedef{N@esmfold.casp16.family}{0.838}
\@namedef{N@esmfold.casp16.len100-300}{0.778}
\@namedef{N@esmfold.casp16.len300-600}{0.816}
\@namedef{N@esmfold.casp16.len<100}{0.590}
\@namedef{N@esmfold.casp16.len>600}{0.636}
\@namedef{N@esmfold.casp16.no_family}{0.670}
\@namedef{N@esmfold.casp16.overall}{0.762}
\@namedef{N@esmfold.casp16.subset}{0.750}
\@namedef{N@esmfold.foldbench334.family}{0.900}
\@namedef{N@esmfold.foldbench334.len100-300}{0.853}
\@namedef{N@esmfold.foldbench334.len300-600}{0.930}
\@namedef{N@esmfold.foldbench334.len<100}{0.801}
\@namedef{N@esmfold.foldbench334.len>600}{0.855}
\@namedef{N@esmfold.foldbench334.no_family}{0.820}
\@namedef{N@esmfold.foldbench334.overall}{0.869}
\@namedef{N@esmfold.foldbench334.subset}{0.841}
\@namedef{N@floor_helix.cameo2025.family}{0.098}
\@namedef{N@floor_helix.cameo2025.len100-300}{0.114}
\@namedef{N@floor_helix.cameo2025.len300-600}{0.078}
\@namedef{N@floor_helix.cameo2025.len<100}{0.191}
\@namedef{N@floor_helix.cameo2025.len>600}{0.053}
\@namedef{N@floor_helix.cameo2025.no_family}{0.115}
\@namedef{N@floor_helix.cameo2025.overall}{0.100}
\@namedef{N@floor_helix.cameo2025.subset}{0.119}
\@namedef{N@floor_helix.casp16.family}{0.132}
\@namedef{N@floor_helix.casp16.len100-300}{0.133}
\@namedef{N@floor_helix.casp16.len300-600}{0.088}
\@namedef{N@floor_helix.casp16.len<100}{0.270}
\@namedef{N@floor_helix.casp16.len>600}{0.053}
\@namedef{N@floor_helix.casp16.no_family}{0.138}
\@namedef{N@floor_helix.casp16.overall}{0.135}
\@namedef{N@floor_helix.casp16.subset}{0.153}
\@namedef{N@floor_helix.foldbench334.family}{0.105}
\@namedef{N@floor_helix.foldbench334.len100-300}{0.126}
\@namedef{N@floor_helix.foldbench334.len300-600}{0.076}
\@namedef{N@floor_helix.foldbench334.len<100}{0.182}
\@namedef{N@floor_helix.foldbench334.len>600}{0.047}
\@namedef{N@floor_helix.foldbench334.no_family}{0.132}
\@namedef{N@floor_helix.foldbench334.overall}{0.115}
\@namedef{N@floor_helix.foldbench334.subset}{0.136}
\@namedef{N@floor_randomwalk.cameo2025.family}{0.135}
\@namedef{N@floor_randomwalk.cameo2025.len100-300}{0.140}
\@namedef{N@floor_randomwalk.cameo2025.len300-600}{0.131}
\@namedef{N@floor_randomwalk.cameo2025.len<100}{0.151}
\@namedef{N@floor_randomwalk.cameo2025.len>600}{0.115}
\@namedef{N@floor_randomwalk.cameo2025.no_family}{0.141}
\@namedef{N@floor_randomwalk.cameo2025.overall}{0.136}
\@namedef{N@floor_randomwalk.cameo2025.subset}{0.138}
\@namedef{N@floor_randomwalk.casp16.family}{0.141}
\@namedef{N@floor_randomwalk.casp16.len100-300}{0.137}
\@namedef{N@floor_randomwalk.casp16.len300-600}{0.137}
\@namedef{N@floor_randomwalk.casp16.len<100}{0.162}
\@namedef{N@floor_randomwalk.casp16.len>600}{0.110}
\@namedef{N@floor_randomwalk.casp16.no_family}{0.135}
\@namedef{N@floor_randomwalk.casp16.overall}{0.139}
\@namedef{N@floor_randomwalk.casp16.subset}{0.141}
\@namedef{N@floor_randomwalk.foldbench334.family}{0.138}
\@namedef{N@floor_randomwalk.foldbench334.len100-300}{0.143}
\@namedef{N@floor_randomwalk.foldbench334.len300-600}{0.133}
\@namedef{N@floor_randomwalk.foldbench334.len<100}{0.152}
\@namedef{N@floor_randomwalk.foldbench334.len>600}{0.126}
\@namedef{N@floor_randomwalk.foldbench334.no_family}{0.144}
\@namedef{N@floor_randomwalk.foldbench334.overall}{0.140}
\@namedef{N@floor_randomwalk.foldbench334.subset}{0.149}
\@namedef{N@llm_claude.cameo2025.subset}{0.196}
\@namedef{N@llm_claude.casp16.subset}{0.196}
\@namedef{N@llm_claude.foldbench334.subset}{0.213}
\@namedef{N@llm_deepseek.cameo2025.subset}{0.147}
\@namedef{N@llm_deepseek.casp16.subset}{0.178}
\@namedef{N@llm_deepseek.foldbench334.subset}{0.158}
\@namedef{N@llm_gemini.cameo2025.subset}{0.162}
\@namedef{N@llm_gemini.casp16.subset}{0.187}
\@namedef{N@llm_gemini.foldbench334.subset}{0.197}
\@namedef{N@llm_gpt.cameo2025.subset}{0.198}
\@namedef{N@llm_gpt.casp16.subset}{0.224}
\@namedef{N@llm_gpt.foldbench334.subset}{0.208}
\@namedef{N@mmlu.biomatrix_1p7b.acc}{0.129}
\@namedef{N@mmlu.biomatrix_1p7b.invalid}{18\%}
\@namedef{N@mmlu.biomatrix_4b.acc}{0.131}
\@namedef{N@mmlu.biomatrix_4b.invalid}{29\%}
\@namedef{N@mmlu.qwen3_1p7b_base.acc}{0.257}
\@namedef{N@mmlu.qwen3_1p7b_base.invalid}{30\%}
\@namedef{N@mmlu.qwen3_1p7b_chat.acc}{0.440}
\@namedef{N@mmlu.qwen3_1p7b_chat.invalid}{0\%}
\@namedef{N@mmlu.qwen3_4b_base.acc}{0.117}
\@namedef{N@mmlu.qwen3_4b_base.invalid}{80\%}
\@namedef{N@mmlu.qwen3_4b_chat.acc}{0.603}
\@namedef{N@mmlu.qwen3_4b_chat.invalid}{0\%}
\@namedef{N@ms.cameo2025.mean}{0.902}
\@namedef{N@ms.cameo2025.medoid}{0.903}
\@namedef{N@ms.cameo2025.medoid_gain}{0.004}
\@namedef{N@ms.cameo2025.oracle}{0.919}
\@namedef{N@ms.cameo2025.oracle_gain}{0.019}
\@namedef{N@ms.cameo2025.single}{0.900}
\@namedef{N@ms.cameo2025.spearman}{0.893}
\@namedef{N@ms.cameo2025.spread}{0.033}
\@namedef{N@ms.cameo2025.worst}{0.886}
\@namedef{N@ms.casp16.mean}{0.633}
\@namedef{N@ms.casp16.medoid}{0.642}
\@namedef{N@ms.casp16.medoid_gain}{0.007}
\@namedef{N@ms.casp16.oracle}{0.679}
\@namedef{N@ms.casp16.oracle_gain}{0.045}
\@namedef{N@ms.casp16.single}{0.635}
\@namedef{N@ms.casp16.spearman}{0.853}
\@namedef{N@ms.casp16.spread}{0.091}
\@namedef{N@ms.casp16.worst}{0.589}
\@namedef{N@ms.foldbench334.mean}{0.808}
\@namedef{N@ms.foldbench334.medoid}{0.814}
\@namedef{N@ms.foldbench334.medoid_gain}{0.006}
\@namedef{N@ms.foldbench334.oracle}{0.837}
\@namedef{N@ms.foldbench334.oracle_gain}{0.030}
\@namedef{N@ms.foldbench334.single}{0.808}
\@namedef{N@ms.foldbench334.spearman}{0.887}
\@namedef{N@ms.foldbench334.spread}{0.064}
\@namedef{N@ms.foldbench334.worst}{0.773}
\@namedef{N@multiflow.cameo2025.family}{0.272}
\@namedef{N@multiflow.cameo2025.len100-300}{0.303}
\@namedef{N@multiflow.cameo2025.len300-600}{0.230}
\@namedef{N@multiflow.cameo2025.len<100}{0.381}
\@namedef{N@multiflow.cameo2025.len>600}{0.188}
\@namedef{N@multiflow.cameo2025.no_family}{0.265}
\@namedef{N@multiflow.cameo2025.overall}{0.272}
\@namedef{N@multiflow.cameo2025.subset}{0.310}
\@namedef{N@multiflow.casp16.family}{0.276}
\@namedef{N@multiflow.casp16.len100-300}{0.258}
\@namedef{N@multiflow.casp16.len300-600}{0.232}
\@namedef{N@multiflow.casp16.len<100}{0.396}
\@namedef{N@multiflow.casp16.len>600}{0.129}
\@namedef{N@multiflow.casp16.no_family}{0.246}
\@namedef{N@multiflow.casp16.overall}{0.262}
\@namedef{N@multiflow.casp16.subset}{0.278}
\@namedef{N@multiflow.foldbench334.family}{0.266}
\@namedef{N@multiflow.foldbench334.len100-300}{0.292}
\@namedef{N@multiflow.foldbench334.len300-600}{0.250}
\@namedef{N@multiflow.foldbench334.len<100}{0.327}
\@namedef{N@multiflow.foldbench334.len>600}{0.181}
\@namedef{N@multiflow.foldbench334.no_family}{0.302}
\@namedef{N@multiflow.foldbench334.overall}{0.280}
\@namedef{N@multiflow.foldbench334.subset}{0.294}
\@namedef{N@opendde_msa.cameo2025.family}{0.959}
\@namedef{N@opendde_msa.cameo2025.len100-300}{0.963}
\@namedef{N@opendde_msa.cameo2025.len300-600}{0.960}
\@namedef{N@opendde_msa.cameo2025.len<100}{0.894}
\@namedef{N@opendde_msa.cameo2025.len>600}{0.894}
\@namedef{N@opendde_msa.cameo2025.no_family}{0.948}
\@namedef{N@opendde_msa.cameo2025.overall}{0.958}
\@namedef{N@opendde_msa.cameo2025.subset}{0.958}
\@namedef{N@opendde_msa.casp16.family}{0.920}
\@namedef{N@opendde_msa.casp16.len100-300}{0.902}
\@namedef{N@opendde_msa.casp16.len300-600}{0.897}
\@namedef{N@opendde_msa.casp16.len<100}{0.710}
\@namedef{N@opendde_msa.casp16.len>600}{0.631}
\@namedef{N@opendde_msa.casp16.no_family}{0.815}
\@namedef{N@opendde_msa.casp16.overall}{0.872}
\@namedef{N@opendde_msa.casp16.subset}{0.869}
\@namedef{N@opendde_msa.foldbench334.family}{0.952}
\@namedef{N@opendde_msa.foldbench334.len100-300}{0.931}
\@namedef{N@opendde_msa.foldbench334.len300-600}{0.967}
\@namedef{N@opendde_msa.foldbench334.len<100}{0.894}
\@namedef{N@opendde_msa.foldbench334.len>600}{0.967}
\@namedef{N@opendde_msa.foldbench334.no_family}{0.917}
\@namedef{N@opendde_msa.foldbench334.overall}{0.938}
\@namedef{N@opendde_msa.foldbench334.subset}{0.934}
\@namedef{N@opendde_single.cameo2025.family}{0.368}
\@namedef{N@opendde_single.cameo2025.len100-300}{0.418}
\@namedef{N@opendde_single.cameo2025.len300-600}{0.303}
\@namedef{N@opendde_single.cameo2025.len<100}{0.571}
\@namedef{N@opendde_single.cameo2025.len>600}{0.296}
\@namedef{N@opendde_single.cameo2025.no_family}{0.398}
\@namedef{N@opendde_single.cameo2025.overall}{0.370}
\@namedef{N@opendde_single.cameo2025.subset}{0.420}
\@namedef{N@opendde_single.casp16.family}{0.370}
\@namedef{N@opendde_single.casp16.len100-300}{0.392}
\@namedef{N@opendde_single.casp16.len300-600}{0.308}
\@namedef{N@opendde_single.casp16.len<100}{0.414}
\@namedef{N@opendde_single.casp16.len>600}{0.162}
\@namedef{N@opendde_single.casp16.no_family}{0.366}
\@namedef{N@opendde_single.casp16.overall}{0.368}
\@namedef{N@opendde_single.casp16.subset}{0.393}
\@namedef{N@opendde_single.foldbench334.family}{0.397}
\@namedef{N@opendde_single.foldbench334.len100-300}{0.454}
\@namedef{N@opendde_single.foldbench334.len300-600}{0.360}
\@namedef{N@opendde_single.foldbench334.len<100}{0.593}
\@namedef{N@opendde_single.foldbench334.len>600}{0.307}
\@namedef{N@opendde_single.foldbench334.no_family}{0.503}
\@namedef{N@opendde_single.foldbench334.overall}{0.438}
\@namedef{N@opendde_single.foldbench334.subset}{0.491}
\@namedef{N@ours_b2.cameo2025.family}{0.918}
\@namedef{N@ours_b2.cameo2025.len100-300}{0.929}
\@namedef{N@ours_b2.cameo2025.len300-600}{0.897}
\@namedef{N@ours_b2.cameo2025.len<100}{0.811}
\@namedef{N@ours_b2.cameo2025.len>600}{0.387}
\@namedef{N@ours_b2.cameo2025.no_family}{0.691}
\@namedef{N@ours_b2.cameo2025.overall}{0.900}
\@namedef{N@ours_b2.cameo2025.subset}{0.909}
\@namedef{N@ours_b2.casp16.family}{0.690}
\@namedef{N@ours_b2.casp16.len100-300}{0.688}
\@namedef{N@ours_b2.casp16.len300-600}{0.542}
\@namedef{N@ours_b2.casp16.len<100}{0.585}
\@namedef{N@ours_b2.casp16.len>600}{0.347}
\@namedef{N@ours_b2.casp16.no_family}{0.567}
\@namedef{N@ours_b2.casp16.overall}{0.635}
\@namedef{N@ours_b2.casp16.subset}{0.667}
\@namedef{N@ours_b2.foldbench334.family}{0.826}
\@namedef{N@ours_b2.foldbench334.len100-300}{0.817}
\@namedef{N@ours_b2.foldbench334.len300-600}{0.817}
\@namedef{N@ours_b2.foldbench334.len<100}{0.821}
\@namedef{N@ours_b2.foldbench334.len>600}{0.536}
\@namedef{N@ours_b2.foldbench334.no_family}{0.779}
\@namedef{N@ours_b2.foldbench334.overall}{0.808}
\@namedef{N@ours_b2.foldbench334.subset}{0.821}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.family.abs}{0.592}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.family.ci}{[$+$0.547, $+$0.637]}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.family.delta}{$+$0.592}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len100-300.abs}{0.566}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len100-300.ci}{[$+$0.504, $+$0.627]}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len100-300.delta}{$+$0.566}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len300-600.abs}{0.627}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len300-600.ci}{[$+$0.563, $+$0.686]}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len300-600.delta}{$+$0.627}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len<100.abs}{0.606}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len<100.ci}{[$+$0.446, $+$0.743]}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.len<100.delta}{$+$0.606}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.no_family.abs}{0.547}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.no_family.ci}{[$+$0.443, $+$0.638]}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.no_family.delta}{$+$0.547}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.overall.abs}{0.589}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.overall.ci}{[$+$0.546, $+$0.630]}
\@namedef{N@ours_b2__vs__biomatrix_4b.cameo2025.overall.delta}{$+$0.589}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.family.abs}{0.524}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.family.ci}{[$+$0.475, $+$0.572]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.family.delta}{$+$0.524}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len100-300.abs}{0.517}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len100-300.ci}{[$+$0.469, $+$0.564]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len100-300.delta}{$+$0.517}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len300-600.abs}{0.423}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len300-600.ci}{[$+$0.364, $+$0.485]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len300-600.delta}{$+$0.423}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len<100.abs}{0.344}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len<100.ci}{[$+$0.219, $+$0.470]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len<100.delta}{$+$0.344}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len>600.abs}{0.282}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len>600.ci}{[$+$0.075, $+$0.600]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.len>600.delta}{$+$0.282}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.no_family.abs}{0.406}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.no_family.ci}{[$+$0.350, $+$0.464]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.no_family.delta}{$+$0.406}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.overall.abs}{0.471}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.overall.ci}{[$+$0.433, $+$0.510]}
\@namedef{N@ours_b2__vs__biomatrix_4b.casp16.overall.delta}{$+$0.471}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.family.abs}{0.671}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.family.ci}{[$+$0.643, $+$0.697]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.family.delta}{$+$0.671}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len100-300.abs}{0.649}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len100-300.ci}{[$+$0.618, $+$0.679]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len100-300.delta}{$+$0.649}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len300-600.abs}{0.682}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len300-600.ci}{[$+$0.648, $+$0.715]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len300-600.delta}{$+$0.682}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len<100.abs}{0.633}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len<100.ci}{[$+$0.561, $+$0.697]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len<100.delta}{$+$0.633}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len>600.abs}{0.434}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len>600.ci}{[$+$0.338, $+$0.535]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.len>600.delta}{$+$0.434}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.no_family.abs}{0.615}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.no_family.ci}{[$+$0.578, $+$0.650]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.no_family.delta}{$+$0.615}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.overall.abs}{0.649}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.overall.ci}{[$+$0.626, $+$0.671]}
\@namedef{N@ours_b2__vs__biomatrix_4b.foldbench334.overall.delta}{$+$0.649}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.family.abs}{0.148}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.family.ci}{[$+$0.121, $+$0.177]}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.family.delta}{$+$0.148}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len100-300.abs}{0.123}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len100-300.ci}{[$+$0.092, $+$0.158]}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len100-300.delta}{$+$0.123}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len300-600.abs}{0.175}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len300-600.ci}{[$+$0.136, $+$0.218]}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len300-600.delta}{$+$0.175}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len<100.abs}{0.143}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len<100.ci}{[$+$0.039, $+$0.279]}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.len<100.delta}{$+$0.143}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.no_family.abs}{0.084}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.no_family.ci}{[$+$0.035, $+$0.131]}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.no_family.delta}{$+$0.084}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.overall.abs}{0.143}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.overall.ci}{[$+$0.118, $+$0.170]}
\@namedef{N@ours_b2__vs__dplm2_650m.cameo2025.overall.delta}{$+$0.143}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.family.abs}{0.104}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.family.ci}{[$+$0.080, $+$0.128]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.family.delta}{$+$0.104}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len100-300.abs}{0.143}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len100-300.ci}{[$+$0.116, $+$0.172]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len100-300.delta}{$+$0.143}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len300-600.abs}{0.107}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len300-600.ci}{[$+$0.075, $+$0.140]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len300-600.delta}{$+$0.107}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len<100.abs}{0.025}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len<100.ci}{[$-$0.011, $+$0.063]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len<100.delta}{$+$0.025}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len>600.abs}{0.044}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len>600.ci}{[$+$0.000, $+$0.121]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.len>600.delta}{$+$0.044}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.no_family.abs}{0.139}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.no_family.ci}{[$+$0.105, $+$0.176]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.no_family.delta}{$+$0.139}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.overall.abs}{0.120}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.overall.ci}{[$+$0.100, $+$0.141]}
\@namedef{N@ours_b2__vs__dplm2_650m.casp16.overall.delta}{$+$0.120}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.family.abs}{0.123}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.family.ci}{[$+$0.104, $+$0.144]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.family.delta}{$+$0.123}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len100-300.abs}{0.183}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len100-300.ci}{[$+$0.158, $+$0.208]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len100-300.delta}{$+$0.183}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len300-600.abs}{0.087}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len300-600.ci}{[$+$0.062, $+$0.112]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len300-600.delta}{$+$0.087}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len<100.abs}{0.200}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len<100.ci}{[$+$0.139, $+$0.270]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len<100.delta}{$+$0.200}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len>600.abs}{0.025}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len>600.ci}{[$-$0.074, $+$0.118]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.len>600.delta}{$+$0.025}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.no_family.abs}{0.197}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.no_family.ci}{[$+$0.162, $+$0.231]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.no_family.delta}{$+$0.197}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.overall.abs}{0.151}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.overall.ci}{[$+$0.133, $+$0.170]}
\@namedef{N@ours_b2__vs__dplm2_650m.foldbench334.overall.delta}{$+$0.151}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.family.abs}{0.067}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.family.ci}{[$+$0.046, $+$0.089]}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.family.delta}{$+$0.067}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len100-300.abs}{0.081}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len100-300.ci}{[$+$0.059, $+$0.107]}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len100-300.delta}{$+$0.081}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len300-600.abs}{0.074}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len300-600.ci}{[$+$0.039, $+$0.111]}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len300-600.delta}{$+$0.074}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len<100.abs}{0.053}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len<100.ci}{[$+$0.024, $+$0.090]}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.len<100.delta}{$+$0.053}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.no_family.abs}{0.134}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.no_family.ci}{[$+$0.097, $+$0.171]}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.no_family.delta}{$+$0.134}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.overall.abs}{0.072}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.overall.ci}{[$+$0.052, $+$0.093]}
\@namedef{N@ours_b2__vs__dplm2p1.cameo2025.overall.delta}{$+$0.072}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.family.abs}{0.076}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.family.ci}{[$+$0.039, $+$0.112]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.family.delta}{$+$0.076}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len100-300.abs}{0.142}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len100-300.ci}{[$+$0.116, $+$0.169]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len100-300.delta}{$+$0.142}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len300-600.abs}{0.026}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len300-600.ci}{[$-$0.036, $+$0.084]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len300-600.delta}{$+$0.026}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len<100.abs}{0.105}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len<100.ci}{[$+$0.014, $+$0.190]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len<100.delta}{$+$0.105}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len>600.abs}{0.013}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len>600.ci}{[$-$0.155, $+$0.068]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.len>600.delta}{$-$0.013}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.no_family.abs}{0.146}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.no_family.ci}{[$+$0.116, $+$0.179]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.no_family.delta}{$+$0.146}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.overall.abs}{0.108}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.overall.ci}{[$+$0.082, $+$0.133]}
\@namedef{N@ours_b2__vs__dplm2p1.casp16.overall.delta}{$+$0.108}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.family.abs}{0.080}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.family.ci}{[$+$0.057, $+$0.104]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.family.delta}{$+$0.080}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len100-300.abs}{0.165}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len100-300.ci}{[$+$0.138, $+$0.192]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len100-300.delta}{$+$0.165}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len300-600.abs}{0.058}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len300-600.ci}{[$+$0.024, $+$0.092]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len300-600.delta}{$+$0.058}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len<100.abs}{0.222}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len<100.ci}{[$+$0.161, $+$0.289]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len<100.delta}{$+$0.222}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len>600.abs}{0.080}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len>600.ci}{[$-$0.212, $+$0.041]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.len>600.delta}{$-$0.080}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.no_family.abs}{0.214}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.no_family.ci}{[$+$0.180, $+$0.248]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.no_family.delta}{$+$0.214}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.overall.abs}{0.132}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.overall.ci}{[$+$0.111, $+$0.152]}
\@namedef{N@ours_b2__vs__dplm2p1.foldbench334.overall.delta}{$+$0.132}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.family.abs}{0.010}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.family.ci}{[$-$0.023, $+$0.003]}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.family.delta}{$-$0.010}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len100-300.abs}{0.000}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len100-300.ci}{[$-$0.014, $+$0.018]}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len100-300.delta}{$-$0.000}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len300-600.abs}{0.025}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len300-600.ci}{[$-$0.044, $-$0.007]}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len300-600.delta}{$-$0.025}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len<100.abs}{0.017}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len<100.ci}{[$-$0.070, $+$0.018]}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.len<100.delta}{$-$0.017}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.no_family.abs}{0.100}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.no_family.ci}{[$-$0.143, $-$0.060]}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.no_family.delta}{$-$0.100}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.overall.abs}{0.017}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.overall.ci}{[$-$0.030, $-$0.004]}
\@namedef{N@ours_b2__vs__esm2_direct.cameo2025.overall.delta}{$-$0.017}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.family.abs}{0.068}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.family.ci}{[$-$0.098, $-$0.039]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.family.delta}{$-$0.068}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len100-300.abs}{0.008}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len100-300.ci}{[$-$0.030, $+$0.015]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len100-300.delta}{$-$0.008}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len300-600.abs}{0.160}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len300-600.ci}{[$-$0.204, $-$0.119]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len300-600.delta}{$-$0.160}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len<100.abs}{0.024}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len<100.ci}{[$-$0.051, $-$0.003]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len<100.delta}{$-$0.024}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len>600.abs}{0.143}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len>600.ci}{[$-$0.375, $-$0.019]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.len>600.delta}{$-$0.143}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.no_family.abs}{0.022}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.no_family.ci}{[$-$0.052, $+$0.007]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.no_family.delta}{$-$0.022}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.overall.abs}{0.047}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.overall.ci}{[$-$0.068, $-$0.026]}
\@namedef{N@ours_b2__vs__esm2_direct.casp16.overall.delta}{$-$0.047}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.family.abs}{0.024}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.family.ci}{[$-$0.039, $-$0.009]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.family.delta}{$-$0.024}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len100-300.abs}{0.004}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len100-300.ci}{[$-$0.015, $+$0.023]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len100-300.delta}{$+$0.004}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len300-600.abs}{0.044}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len300-600.ci}{[$-$0.068, $-$0.021]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len300-600.delta}{$-$0.044}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len<100.abs}{0.013}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len<100.ci}{[$-$0.064, $+$0.043]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len<100.delta}{$-$0.013}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len>600.abs}{0.062}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len>600.ci}{[$-$0.146, $+$0.019]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.len>600.delta}{$-$0.062}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.no_family.abs}{0.002}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.no_family.ci}{[$-$0.026, $+$0.032]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.no_family.delta}{$+$0.002}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.overall.abs}{0.014}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.overall.ci}{[$-$0.028, $+$0.000]}
\@namedef{N@ours_b2__vs__esm2_direct.foldbench334.overall.delta}{$-$0.014}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.family.abs}{0.056}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.family.ci}{[$+$0.029, $+$0.084]}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.family.delta}{$+$0.056}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len100-300.abs}{0.059}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len100-300.ci}{[$+$0.029, $+$0.094]}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len100-300.delta}{$+$0.059}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len300-600.abs}{0.047}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len300-600.ci}{[$+$0.008, $+$0.090]}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len300-600.delta}{$+$0.047}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len<100.abs}{0.028}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len<100.ci}{[$+$0.003, $+$0.059]}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.len<100.delta}{$+$0.028}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.no_family.abs}{0.048}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.no_family.ci}{[$-$0.085, $-$0.013]}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.no_family.delta}{$-$0.048}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.overall.abs}{0.048}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.overall.ci}{[$+$0.023, $+$0.074]}
\@namedef{N@ours_b2__vs__esm3_open.cameo2025.overall.delta}{$+$0.048}
\@namedef{N@ours_b2__vs__esm3_open.casp16.family.abs}{0.035}
\@namedef{N@ours_b2__vs__esm3_open.casp16.family.ci}{[$-$0.068, $-$0.004]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.family.delta}{$-$0.035}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len100-300.abs}{0.025}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len100-300.ci}{[$+$0.006, $+$0.044]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len100-300.delta}{$+$0.025}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len300-600.abs}{0.077}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len300-600.ci}{[$-$0.142, $-$0.017]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len300-600.delta}{$-$0.077}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len<100.abs}{0.013}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len<100.ci}{[$-$0.056, $+$0.022]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len<100.delta}{$-$0.013}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len>600.abs}{0.181}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len>600.ci}{[$-$0.392, $-$0.063]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.len>600.delta}{$-$0.181}
\@namedef{N@ours_b2__vs__esm3_open.casp16.no_family.abs}{0.024}
\@namedef{N@ours_b2__vs__esm3_open.casp16.no_family.ci}{[$-$0.001, $+$0.049]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.no_family.delta}{$+$0.024}
\@namedef{N@ours_b2__vs__esm3_open.casp16.overall.abs}{0.008}
\@namedef{N@ours_b2__vs__esm3_open.casp16.overall.ci}{[$-$0.031, $+$0.013]}
\@namedef{N@ours_b2__vs__esm3_open.casp16.overall.delta}{$-$0.008}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.family.abs}{0.003}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.family.ci}{[$-$0.028, $+$0.022]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.family.delta}{$-$0.003}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len100-300.abs}{0.061}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len100-300.ci}{[$+$0.035, $+$0.087]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len100-300.delta}{$+$0.061}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len300-600.abs}{0.058}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len300-600.ci}{[$-$0.088, $-$0.026]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len300-600.delta}{$-$0.058}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len<100.abs}{0.112}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len<100.ci}{[$+$0.048, $+$0.185]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len<100.delta}{$+$0.112}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len>600.abs}{0.270}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len>600.ci}{[$-$0.400, $-$0.146]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.len>600.delta}{$-$0.270}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.no_family.abs}{0.059}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.no_family.ci}{[$+$0.021, $+$0.097]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.no_family.delta}{$+$0.059}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.overall.abs}{0.021}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.overall.ci}{[$-$0.000, $+$0.042]}
\@namedef{N@ours_b2__vs__esm3_open.foldbench334.overall.delta}{$+$0.021}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.family.abs}{0.009}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.family.ci}{[$-$0.014, $+$0.033]}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.family.delta}{$+$0.009}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len100-300.abs}{0.018}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len100-300.ci}{[$-$0.008, $+$0.049]}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len100-300.delta}{$+$0.018}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len300-600.abs}{0.015}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len300-600.ci}{[$-$0.049, $+$0.021]}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len300-600.delta}{$-$0.015}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len<100.abs}{0.028}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len<100.ci}{[$-$0.105, $+$0.023]}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.len<100.delta}{$-$0.028}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.no_family.abs}{0.164}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.no_family.ci}{[$-$0.223, $-$0.112]}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.no_family.delta}{$-$0.164}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.overall.abs}{0.005}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.overall.ci}{[$-$0.028, $+$0.019]}
\@namedef{N@ours_b2__vs__esmfold.cameo2025.overall.delta}{$-$0.005}
\@namedef{N@ours_b2__vs__esmfold.casp16.family.abs}{0.148}
\@namedef{N@ours_b2__vs__esmfold.casp16.family.ci}{[$-$0.188, $-$0.110]}
\@namedef{N@ours_b2__vs__esmfold.casp16.family.delta}{$-$0.148}
\@namedef{N@ours_b2__vs__esmfold.casp16.len100-300.abs}{0.090}
\@namedef{N@ours_b2__vs__esmfold.casp16.len100-300.ci}{[$-$0.118, $-$0.063]}
\@namedef{N@ours_b2__vs__esmfold.casp16.len100-300.delta}{$-$0.090}
\@namedef{N@ours_b2__vs__esmfold.casp16.len300-600.abs}{0.274}
\@namedef{N@ours_b2__vs__esmfold.casp16.len300-600.ci}{[$-$0.328, $-$0.219]}
\@namedef{N@ours_b2__vs__esmfold.casp16.len300-600.delta}{$-$0.274}
\@namedef{N@ours_b2__vs__esmfold.casp16.len<100.abs}{0.005}
\@namedef{N@ours_b2__vs__esmfold.casp16.len<100.ci}{[$-$0.023, $+$0.012]}
\@namedef{N@ours_b2__vs__esmfold.casp16.len<100.delta}{$-$0.005}
\@namedef{N@ours_b2__vs__esmfold.casp16.len>600.abs}{0.289}
\@namedef{N@ours_b2__vs__esmfold.casp16.len>600.ci}{[$-$0.481, $-$0.130]}
\@namedef{N@ours_b2__vs__esmfold.casp16.len>600.delta}{$-$0.289}
\@namedef{N@ours_b2__vs__esmfold.casp16.no_family.abs}{0.103}
\@namedef{N@ours_b2__vs__esmfold.casp16.no_family.ci}{[$-$0.137, $-$0.071]}
\@namedef{N@ours_b2__vs__esmfold.casp16.no_family.delta}{$-$0.103}
\@namedef{N@ours_b2__vs__esmfold.casp16.overall.abs}{0.128}
\@namedef{N@ours_b2__vs__esmfold.casp16.overall.ci}{[$-$0.154, $-$0.102]}
\@namedef{N@ours_b2__vs__esmfold.casp16.overall.delta}{$-$0.128}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.family.abs}{0.075}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.family.ci}{[$-$0.097, $-$0.053]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.family.delta}{$-$0.075}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len100-300.abs}{0.036}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len100-300.ci}{[$-$0.057, $-$0.013]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len100-300.delta}{$-$0.036}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len300-600.abs}{0.112}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len300-600.ci}{[$-$0.142, $-$0.084]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len300-600.delta}{$-$0.112}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len<100.abs}{0.019}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len<100.ci}{[$-$0.044, $+$0.086]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len<100.delta}{$+$0.019}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len>600.abs}{0.319}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len>600.ci}{[$-$0.435, $-$0.210]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.len>600.delta}{$-$0.319}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.no_family.abs}{0.041}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.no_family.ci}{[$-$0.074, $-$0.008]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.no_family.delta}{$-$0.041}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.overall.abs}{0.062}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.overall.ci}{[$-$0.080, $-$0.043]}
\@namedef{N@ours_b2__vs__esmfold.foldbench334.overall.delta}{$-$0.062}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.family.abs}{0.551}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.family.ci}{[$+$0.523, $+$0.578]}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.family.delta}{$+$0.551}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len100-300.abs}{0.512}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len100-300.ci}{[$+$0.471, $+$0.549]}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len100-300.delta}{$+$0.512}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len300-600.abs}{0.594}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len300-600.ci}{[$+$0.559, $+$0.630]}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len300-600.delta}{$+$0.594}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len<100.abs}{0.240}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len<100.ci}{[$+$0.074, $+$0.435]}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.len<100.delta}{$+$0.240}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.no_family.abs}{0.293}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.no_family.ci}{[$+$0.169, $+$0.418]}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.no_family.delta}{$+$0.293}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.overall.abs}{0.530}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.overall.ci}{[$+$0.501, $+$0.559]}
\@namedef{N@ours_b2__vs__opendde_single.cameo2025.overall.delta}{$+$0.530}
\@namedef{N@ours_b2__vs__opendde_single.casp16.family.abs}{0.320}
\@namedef{N@ours_b2__vs__opendde_single.casp16.family.ci}{[$+$0.270, $+$0.371]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.family.delta}{$+$0.320}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len100-300.abs}{0.297}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len100-300.ci}{[$+$0.246, $+$0.344]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len100-300.delta}{$+$0.297}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len300-600.abs}{0.234}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len300-600.ci}{[$+$0.182, $+$0.289]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len300-600.delta}{$+$0.234}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len<100.abs}{0.172}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len<100.ci}{[$+$0.060, $+$0.304]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len<100.delta}{$+$0.172}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len>600.abs}{0.185}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len>600.ci}{[$+$0.018, $+$0.470]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.len>600.delta}{$+$0.185}
\@namedef{N@ours_b2__vs__opendde_single.casp16.no_family.abs}{0.201}
\@namedef{N@ours_b2__vs__opendde_single.casp16.no_family.ci}{[$+$0.147, $+$0.256]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.no_family.delta}{$+$0.201}
\@namedef{N@ours_b2__vs__opendde_single.casp16.overall.abs}{0.266}
\@namedef{N@ours_b2__vs__opendde_single.casp16.overall.ci}{[$+$0.229, $+$0.305]}
\@namedef{N@ours_b2__vs__opendde_single.casp16.overall.delta}{$+$0.266}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.family.abs}{0.428}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.family.ci}{[$+$0.395, $+$0.461]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.family.delta}{$+$0.428}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len100-300.abs}{0.363}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len100-300.ci}{[$+$0.318, $+$0.407]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len100-300.delta}{$+$0.363}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len300-600.abs}{0.457}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len300-600.ci}{[$+$0.418, $+$0.496]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len300-600.delta}{$+$0.457}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len<100.abs}{0.228}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len<100.ci}{[$+$0.130, $+$0.323]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len<100.delta}{$+$0.228}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len>600.abs}{0.228}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len>600.ci}{[$+$0.098, $+$0.345]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.len>600.delta}{$+$0.228}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.no_family.abs}{0.276}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.no_family.ci}{[$+$0.223, $+$0.329]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.no_family.delta}{$+$0.276}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.overall.abs}{0.370}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.overall.ci}{[$+$0.340, $+$0.399]}
\@namedef{N@ours_b2__vs__opendde_single.foldbench334.overall.delta}{$+$0.370}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.family.abs}{0.055}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.family.ci}{[$+$0.042, $+$0.068]}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.family.delta}{$+$0.055}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len100-300.abs}{0.014}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len100-300.ci}{[$+$0.008, $+$0.021]}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len100-300.delta}{$+$0.014}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len300-600.abs}{0.104}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len300-600.ci}{[$+$0.082, $+$0.127]}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len300-600.delta}{$+$0.104}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len<100.abs}{0.028}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len<100.ci}{[$+$0.001, $+$0.063]}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.len<100.delta}{$+$0.028}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.no_family.abs}{0.060}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.no_family.ci}{[$+$0.029, $+$0.090]}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.no_family.delta}{$+$0.060}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.overall.abs}{0.055}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.overall.ci}{[$+$0.043, $+$0.068]}
\@namedef{N@ours_b2__vs__ours_joint.cameo2025.overall.delta}{$+$0.055}
\@namedef{N@ours_b2__vs__ours_joint.casp16.family.abs}{0.042}
\@namedef{N@ours_b2__vs__ours_joint.casp16.family.ci}{[$+$0.023, $+$0.063]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.family.delta}{$+$0.042}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len100-300.abs}{0.057}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len100-300.ci}{[$+$0.038, $+$0.076]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len100-300.delta}{$+$0.057}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len300-600.abs}{0.054}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len300-600.ci}{[$+$0.025, $+$0.084]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len300-600.delta}{$+$0.054}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len<100.abs}{0.004}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len<100.ci}{[$-$0.012, $+$0.022]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len<100.delta}{$+$0.004}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len>600.abs}{0.117}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len>600.ci}{[$+$0.007, $+$0.294]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.len>600.delta}{$+$0.117}
\@namedef{N@ours_b2__vs__ours_joint.casp16.no_family.abs}{0.065}
\@namedef{N@ours_b2__vs__ours_joint.casp16.no_family.ci}{[$+$0.042, $+$0.090]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.no_family.delta}{$+$0.065}
\@namedef{N@ours_b2__vs__ours_joint.casp16.overall.abs}{0.052}
\@namedef{N@ours_b2__vs__ours_joint.casp16.overall.ci}{[$+$0.038, $+$0.068]}
\@namedef{N@ours_b2__vs__ours_joint.casp16.overall.delta}{$+$0.052}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.family.abs}{0.064}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.family.ci}{[$+$0.052, $+$0.077]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.family.delta}{$+$0.064}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len100-300.abs}{0.038}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len100-300.ci}{[$+$0.026, $+$0.051]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len100-300.delta}{$+$0.038}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len300-600.abs}{0.119}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len300-600.ci}{[$+$0.097, $+$0.141]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len300-600.delta}{$+$0.119}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len<100.abs}{0.016}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len<100.ci}{[$+$0.001, $+$0.034]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len<100.delta}{$+$0.016}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len>600.abs}{0.167}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len>600.ci}{[$+$0.091, $+$0.260]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.len>600.delta}{$+$0.167}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.no_family.abs}{0.062}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.no_family.ci}{[$+$0.042, $+$0.083]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.no_family.delta}{$+$0.062}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.overall.abs}{0.063}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.overall.ci}{[$+$0.052, $+$0.075]}
\@namedef{N@ours_b2__vs__ours_joint.foldbench334.overall.delta}{$+$0.063}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.family.abs}{0.103}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.family.ci}{[$+$0.083, $+$0.125]}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.family.delta}{$+$0.103}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len100-300.abs}{0.088}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len100-300.ci}{[$+$0.064, $+$0.116]}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len100-300.delta}{$+$0.088}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len300-600.abs}{0.120}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len300-600.ci}{[$+$0.090, $+$0.153]}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len300-600.delta}{$+$0.120}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len<100.abs}{0.075}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len<100.ci}{[$+$0.033, $+$0.120]}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.len<100.delta}{$+$0.075}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.no_family.abs}{0.070}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.no_family.ci}{[$+$0.045, $+$0.097]}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.no_family.delta}{$+$0.070}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.overall.abs}{0.100}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.overall.ci}{[$+$0.081, $+$0.120]}
\@namedef{N@ours_b2__vs__ours_token.cameo2025.overall.delta}{$+$0.100}
\@namedef{N@ours_b2__vs__ours_token.casp16.family.abs}{0.026}
\@namedef{N@ours_b2__vs__ours_token.casp16.family.ci}{[$+$0.006, $+$0.046]}
\@namedef{N@ours_b2__vs__ours_token.casp16.family.delta}{$+$0.026}
\@namedef{N@ours_b2__vs__ours_token.casp16.len100-300.abs}{0.083}
\@namedef{N@ours_b2__vs__ours_token.casp16.len100-300.ci}{[$+$0.061, $+$0.106]}
\@namedef{N@ours_b2__vs__ours_token.casp16.len100-300.delta}{$+$0.083}
\@namedef{N@ours_b2__vs__ours_token.casp16.len300-600.abs}{0.034}
\@namedef{N@ours_b2__vs__ours_token.casp16.len300-600.ci}{[$-$0.008, $+$0.075]}
\@namedef{N@ours_b2__vs__ours_token.casp16.len300-600.delta}{$+$0.034}
\@namedef{N@ours_b2__vs__ours_token.casp16.len<100.abs}{0.025}
\@namedef{N@ours_b2__vs__ours_token.casp16.len<100.ci}{[$+$0.004, $+$0.048]}
\@namedef{N@ours_b2__vs__ours_token.casp16.len<100.delta}{$+$0.025}
\@namedef{N@ours_b2__vs__ours_token.casp16.len>600.abs}{0.072}
\@namedef{N@ours_b2__vs__ours_token.casp16.len>600.ci}{[$+$0.010, $+$0.173]}
\@namedef{N@ours_b2__vs__ours_token.casp16.len>600.delta}{$+$0.072}
\@namedef{N@ours_b2__vs__ours_token.casp16.no_family.abs}{0.114}
\@namedef{N@ours_b2__vs__ours_token.casp16.no_family.ci}{[$+$0.088, $+$0.143]}
\@namedef{N@ours_b2__vs__ours_token.casp16.no_family.delta}{$+$0.114}
\@namedef{N@ours_b2__vs__ours_token.casp16.overall.abs}{0.066}
\@namedef{N@ours_b2__vs__ours_token.casp16.overall.ci}{[$+$0.048, $+$0.084]}
\@namedef{N@ours_b2__vs__ours_token.casp16.overall.delta}{$+$0.066}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.family.abs}{0.126}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.family.ci}{[$+$0.109, $+$0.143]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.family.delta}{$+$0.126}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len100-300.abs}{0.164}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len100-300.ci}{[$+$0.142, $+$0.188]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len100-300.delta}{$+$0.164}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len300-600.abs}{0.109}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len300-600.ci}{[$+$0.086, $+$0.134]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len300-600.delta}{$+$0.109}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len<100.abs}{0.171}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len<100.ci}{[$+$0.105, $+$0.244]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len<100.delta}{$+$0.171}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len>600.abs}{0.113}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len>600.ci}{[$+$0.021, $+$0.210]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.len>600.delta}{$+$0.113}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.no_family.abs}{0.182}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.no_family.ci}{[$+$0.148, $+$0.216]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.no_family.delta}{$+$0.182}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.overall.abs}{0.147}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.overall.ci}{[$+$0.130, $+$0.165]}
\@namedef{N@ours_b2__vs__ours_token.foldbench334.overall.delta}{$+$0.147}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.family.abs}{0.022}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.family.ci}{[$-$0.002, $+$0.046]}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.family.delta}{$+$0.022}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len100-300.abs}{0.094}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len100-300.ci}{[$+$0.057, $+$0.133]}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len100-300.delta}{$+$0.094}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len300-600.abs}{0.028}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len300-600.ci}{[$-$0.006, $+$0.065]}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len300-600.delta}{$+$0.028}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len<100.abs}{0.048}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len<100.ci}{[$-$0.166, $+$0.217]}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.len<100.delta}{$+$0.048}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.no_family.abs}{0.449}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.no_family.ci}{[$+$0.343, $+$0.566]}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.no_family.delta}{$+$0.449}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.overall.abs}{0.056}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.overall.ci}{[$+$0.028, $+$0.085]}
\@namedef{N@ours_b2__vs__retrieval.cameo2025.overall.delta}{$+$0.056}
\@namedef{N@ours_b2__vs__retrieval.casp16.family.abs}{0.106}
\@namedef{N@ours_b2__vs__retrieval.casp16.family.ci}{[$-$0.165, $-$0.047]}
\@namedef{N@ours_b2__vs__retrieval.casp16.family.delta}{$-$0.106}
\@namedef{N@ours_b2__vs__retrieval.casp16.len100-300.abs}{0.224}
\@namedef{N@ours_b2__vs__retrieval.casp16.len100-300.ci}{[$+$0.149, $+$0.299]}
\@namedef{N@ours_b2__vs__retrieval.casp16.len100-300.delta}{$+$0.224}
\@namedef{N@ours_b2__vs__retrieval.casp16.len300-600.abs}{0.011}
\@namedef{N@ours_b2__vs__retrieval.casp16.len300-600.ci}{[$-$0.143, $+$0.126]}
\@namedef{N@ours_b2__vs__retrieval.casp16.len300-600.delta}{$-$0.011}
\@namedef{N@ours_b2__vs__retrieval.casp16.len<100.abs}{0.217}
\@namedef{N@ours_b2__vs__retrieval.casp16.len<100.ci}{[$-$0.019, $+$0.435]}
\@namedef{N@ours_b2__vs__retrieval.casp16.len<100.delta}{$+$0.217}
\@namedef{N@ours_b2__vs__retrieval.casp16.len>600.abs}{0.019}
\@namedef{N@ours_b2__vs__retrieval.casp16.len>600.ci}{[$-$0.184, $+$0.154]}
\@namedef{N@ours_b2__vs__retrieval.casp16.len>600.delta}{$+$0.019}
\@namedef{N@ours_b2__vs__retrieval.casp16.no_family.abs}{0.495}
\@namedef{N@ours_b2__vs__retrieval.casp16.no_family.ci}{[$+$0.434, $+$0.557]}
\@namedef{N@ours_b2__vs__retrieval.casp16.no_family.delta}{$+$0.495}
\@namedef{N@ours_b2__vs__retrieval.casp16.overall.abs}{0.165}
\@namedef{N@ours_b2__vs__retrieval.casp16.overall.ci}{[$+$0.101, $+$0.229]}
\@namedef{N@ours_b2__vs__retrieval.casp16.overall.delta}{$+$0.165}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.family.abs}{0.037}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.family.ci}{[$-$0.001, $+$0.075]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.family.delta}{$+$0.037}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len100-300.abs}{0.333}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len100-300.ci}{[$+$0.274, $+$0.392]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len100-300.delta}{$+$0.333}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len300-600.abs}{0.105}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len300-600.ci}{[$+$0.041, $+$0.172]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len300-600.delta}{$+$0.105}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len<100.abs}{0.385}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len<100.ci}{[$+$0.276, $+$0.494]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len<100.delta}{$+$0.385}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len>600.abs}{0.023}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len>600.ci}{[$-$0.269, $+$0.224]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.len>600.delta}{$-$0.023}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.no_family.abs}{0.620}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.no_family.ci}{[$+$0.570, $+$0.668]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.no_family.delta}{$+$0.620}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.overall.abs}{0.261}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.overall.ci}{[$+$0.218, $+$0.304]}
\@namedef{N@ours_b2__vs__retrieval.foldbench334.overall.delta}{$+$0.261}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.family.abs}{0.011}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.family.ci}{[$-$0.004, $+$0.027]}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.family.delta}{$+$0.011}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len100-300.abs}{0.016}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len100-300.ci}{[$+$0.001, $+$0.036]}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len100-300.delta}{$+$0.016}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len300-600.abs}{0.001}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len300-600.ci}{[$-$0.024, $+$0.025]}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len300-600.delta}{$-$0.001}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len<100.abs}{0.015}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len<100.ci}{[$+$0.005, $+$0.026]}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.len<100.delta}{$+$0.015}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.no_family.abs}{0.060}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.no_family.ci}{[$-$0.094, $-$0.031]}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.no_family.delta}{$-$0.060}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.overall.abs}{0.005}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.overall.ci}{[$-$0.009, $+$0.021]}
\@namedef{N@ours_b2__vs__sf100m_official.cameo2025.overall.delta}{$+$0.005}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.family.abs}{0.043}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.family.ci}{[$-$0.070, $-$0.018]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.family.delta}{$-$0.043}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len100-300.abs}{0.000}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len100-300.ci}{[$-$0.019, $+$0.019]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len100-300.delta}{$+$0.000}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len300-600.abs}{0.100}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len300-600.ci}{[$-$0.148, $-$0.055]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len300-600.delta}{$-$0.100}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len<100.abs}{0.013}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len<100.ci}{[$-$0.007, $+$0.033]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len<100.delta}{$+$0.013}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len>600.abs}{0.132}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len>600.ci}{[$-$0.323, $-$0.026]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.len>600.delta}{$-$0.132}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.no_family.abs}{0.003}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.no_family.ci}{[$-$0.028, $+$0.021]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.no_family.delta}{$-$0.003}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.overall.abs}{0.025}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.overall.ci}{[$-$0.043, $-$0.007]}
\@namedef{N@ours_b2__vs__sf100m_official.casp16.overall.delta}{$-$0.025}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.family.abs}{0.013}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.family.ci}{[$-$0.032, $+$0.005]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.family.delta}{$-$0.013}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len100-300.abs}{0.044}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len100-300.ci}{[$+$0.025, $+$0.064]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len100-300.delta}{$+$0.044}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len300-600.abs}{0.048}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len300-600.ci}{[$-$0.075, $-$0.022]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len300-600.delta}{$-$0.048}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len<100.abs}{0.084}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len<100.ci}{[$+$0.030, $+$0.148]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len<100.delta}{$+$0.084}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len>600.abs}{0.205}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len>600.ci}{[$-$0.326, $-$0.097]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.len>600.delta}{$-$0.205}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.no_family.abs}{0.054}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.no_family.ci}{[$+$0.023, $+$0.087]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.no_family.delta}{$+$0.054}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.overall.abs}{0.013}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.overall.ci}{[$-$0.004, $+$0.030]}
\@namedef{N@ours_b2__vs__sf100m_official.foldbench334.overall.delta}{$+$0.013}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.family.abs}{0.030}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.family.ci}{[$-$0.044, $-$0.015]}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.family.delta}{$-$0.030}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len100-300.abs}{0.010}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len100-300.ci}{[$-$0.023, $+$0.007]}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len100-300.delta}{$-$0.010}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len300-600.abs}{0.057}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len300-600.ci}{[$-$0.078, $-$0.038]}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len300-600.delta}{$-$0.057}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len<100.abs}{0.020}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len<100.ci}{[$-$0.092, $+$0.023]}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.len<100.delta}{$-$0.020}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.no_family.abs}{0.130}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.no_family.ci}{[$-$0.181, $-$0.084]}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.no_family.delta}{$-$0.130}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.overall.abs}{0.038}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.overall.ci}{[$-$0.052, $-$0.023]}
\@namedef{N@ours_b2__vs__sf3b_official.cameo2025.overall.delta}{$-$0.038}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.family.abs}{0.100}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.family.ci}{[$-$0.136, $-$0.065]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.family.delta}{$-$0.100}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len100-300.abs}{0.023}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len100-300.ci}{[$-$0.044, $-$0.002]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len100-300.delta}{$-$0.023}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len300-600.abs}{0.218}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len300-600.ci}{[$-$0.276, $-$0.164]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len300-600.delta}{$-$0.218}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len<100.abs}{0.005}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len<100.ci}{[$-$0.025, $+$0.017]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len<100.delta}{$-$0.005}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len>600.abs}{0.200}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len>600.ci}{[$-$0.421, $-$0.063]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.len>600.delta}{$-$0.200}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.no_family.abs}{0.033}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.no_family.ci}{[$-$0.060, $-$0.008]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.no_family.delta}{$-$0.033}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.overall.abs}{0.070}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.overall.ci}{[$-$0.093, $-$0.047]}
\@namedef{N@ours_b2__vs__sf3b_official.casp16.overall.delta}{$-$0.070}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.family.abs}{0.058}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.family.ci}{[$-$0.080, $-$0.039]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.family.delta}{$-$0.058}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len100-300.abs}{0.006}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len100-300.ci}{[$-$0.027, $+$0.015]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len100-300.delta}{$-$0.006}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len300-600.abs}{0.097}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len300-600.ci}{[$-$0.127, $-$0.067]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len300-600.delta}{$-$0.097}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len<100.abs}{0.065}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len<100.ci}{[$+$0.013, $+$0.129]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len<100.delta}{$+$0.065}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len>600.abs}{0.285}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len>600.ci}{[$-$0.396, $-$0.182]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.len>600.delta}{$-$0.285}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.no_family.abs}{0.005}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.no_family.ci}{[$-$0.027, $+$0.038]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.no_family.delta}{$+$0.005}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.overall.abs}{0.034}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.overall.ci}{[$-$0.052, $-$0.016]}
\@namedef{N@ours_b2__vs__sf3b_official.foldbench334.overall.delta}{$-$0.034}
\@namedef{N@ours_joint.cameo2025.family}{0.863}
\@namedef{N@ours_joint.cameo2025.len100-300}{0.915}
\@namedef{N@ours_joint.cameo2025.len300-600}{0.793}
\@namedef{N@ours_joint.cameo2025.len<100}{0.783}
\@namedef{N@ours_joint.cameo2025.len>600}{0.324}
\@namedef{N@ours_joint.cameo2025.no_family}{0.631}
\@namedef{N@ours_joint.cameo2025.overall}{0.845}
\@namedef{N@ours_joint.cameo2025.subset}{0.894}
\@namedef{N@ours_joint.casp16.family}{0.648}
\@namedef{N@ours_joint.casp16.len100-300}{0.632}
\@namedef{N@ours_joint.casp16.len300-600}{0.488}
\@namedef{N@ours_joint.casp16.len<100}{0.581}
\@namedef{N@ours_joint.casp16.len>600}{0.229}
\@namedef{N@ours_joint.casp16.no_family}{0.502}
\@namedef{N@ours_joint.casp16.overall}{0.582}
\@namedef{N@ours_joint.casp16.subset}{0.621}
\@namedef{N@ours_joint.foldbench334.family}{0.761}
\@namedef{N@ours_joint.foldbench334.len100-300}{0.779}
\@namedef{N@ours_joint.foldbench334.len300-600}{0.699}
\@namedef{N@ours_joint.foldbench334.len<100}{0.805}
\@namedef{N@ours_joint.foldbench334.len>600}{0.369}
\@namedef{N@ours_joint.foldbench334.no_family}{0.717}
\@namedef{N@ours_joint.foldbench334.overall}{0.744}
\@namedef{N@ours_joint.foldbench334.subset}{0.783}
\@namedef{N@ours_token.cameo2025.family}{0.815}
\@namedef{N@ours_token.cameo2025.len100-300}{0.841}
\@namedef{N@ours_token.cameo2025.len300-600}{0.777}
\@namedef{N@ours_token.cameo2025.len<100}{0.735}
\@namedef{N@ours_token.cameo2025.len>600}{0.363}
\@namedef{N@ours_token.cameo2025.no_family}{0.621}
\@namedef{N@ours_token.cameo2025.overall}{0.800}
\@namedef{N@ours_token.casp16.family}{0.664}
\@namedef{N@ours_token.casp16.len100-300}{0.606}
\@namedef{N@ours_token.casp16.len300-600}{0.508}
\@namedef{N@ours_token.casp16.len<100}{0.560}
\@namedef{N@ours_token.casp16.len>600}{0.275}
\@namedef{N@ours_token.casp16.no_family}{0.453}
\@namedef{N@ours_token.casp16.overall}{0.569}
\@namedef{N@ours_token.foldbench334.family}{0.700}
\@namedef{N@ours_token.foldbench334.len100-300}{0.653}
\@namedef{N@ours_token.foldbench334.len300-600}{0.708}
\@namedef{N@ours_token.foldbench334.len<100}{0.650}
\@namedef{N@ours_token.foldbench334.len>600}{0.423}
\@namedef{N@ours_token.foldbench334.no_family}{0.597}
\@namedef{N@ours_token.foldbench334.overall}{0.660}
\@namedef{N@retrieval.cameo2025.family}{0.896}
\@namedef{N@retrieval.cameo2025.len100-300}{0.835}
\@namedef{N@retrieval.cameo2025.len300-600}{0.868}
\@namedef{N@retrieval.cameo2025.len<100}{0.762}
\@namedef{N@retrieval.cameo2025.len>600}{0.659}
\@namedef{N@retrieval.cameo2025.no_family}{0.242}
\@namedef{N@retrieval.cameo2025.overall}{0.844}
\@namedef{N@retrieval.cameo2025.subset}{0.767}
\@namedef{N@retrieval.casp16.family}{0.797}
\@namedef{N@retrieval.casp16.len100-300}{0.464}
\@namedef{N@retrieval.casp16.len300-600}{0.553}
\@namedef{N@retrieval.casp16.len<100}{0.368}
\@namedef{N@retrieval.casp16.len>600}{0.327}
\@namedef{N@retrieval.casp16.no_family}{0.072}
\@namedef{N@retrieval.casp16.overall}{0.469}
\@namedef{N@retrieval.casp16.subset}{0.478}
\@namedef{N@retrieval.foldbench334.family}{0.788}
\@namedef{N@retrieval.foldbench334.len100-300}{0.484}
\@namedef{N@retrieval.foldbench334.len300-600}{0.712}
\@namedef{N@retrieval.foldbench334.len<100}{0.436}
\@namedef{N@retrieval.foldbench334.len>600}{0.559}
\@namedef{N@retrieval.foldbench334.no_family}{0.159}
\@namedef{N@retrieval.foldbench334.overall}{0.547}
\@namedef{N@retrieval.foldbench334.subset}{0.536}
\@namedef{N@sf100m_official.cameo2025.family}{0.907}
\@namedef{N@sf100m_official.cameo2025.len100-300}{0.913}
\@namedef{N@sf100m_official.cameo2025.len300-600}{0.898}
\@namedef{N@sf100m_official.cameo2025.len<100}{0.795}
\@namedef{N@sf100m_official.cameo2025.len>600}{0.555}
\@namedef{N@sf100m_official.cameo2025.no_family}{0.752}
\@namedef{N@sf100m_official.cameo2025.overall}{0.895}
\@namedef{N@sf100m_official.cameo2025.subset}{0.896}
\@namedef{N@sf100m_official.casp16.family}{0.733}
\@namedef{N@sf100m_official.casp16.len100-300}{0.688}
\@namedef{N@sf100m_official.casp16.len300-600}{0.641}
\@namedef{N@sf100m_official.casp16.len<100}{0.572}
\@namedef{N@sf100m_official.casp16.len>600}{0.479}
\@namedef{N@sf100m_official.casp16.no_family}{0.570}
\@namedef{N@sf100m_official.casp16.overall}{0.659}
\@namedef{N@sf100m_official.casp16.subset}{0.669}
\@namedef{N@sf100m_official.foldbench334.family}{0.839}
\@namedef{N@sf100m_official.foldbench334.len100-300}{0.774}
\@namedef{N@sf100m_official.foldbench334.len300-600}{0.866}
\@namedef{N@sf100m_official.foldbench334.len<100}{0.737}
\@namedef{N@sf100m_official.foldbench334.len>600}{0.741}
\@namedef{N@sf100m_official.foldbench334.no_family}{0.724}
\@namedef{N@sf100m_official.foldbench334.overall}{0.795}
\@namedef{N@sf100m_official.foldbench334.subset}{0.769}
\@namedef{N@sf3b_official.cameo2025.family}{0.948}
\@namedef{N@sf3b_official.cameo2025.len100-300}{0.939}
\@namedef{N@sf3b_official.cameo2025.len300-600}{0.954}
\@namedef{N@sf3b_official.cameo2025.len<100}{0.831}
\@namedef{N@sf3b_official.cameo2025.len>600}{0.719}
\@namedef{N@sf3b_official.cameo2025.no_family}{0.822}
\@namedef{N@sf3b_official.cameo2025.overall}{0.938}
\@namedef{N@sf3b_official.cameo2025.subset}{0.922}
\@namedef{N@sf3b_official.casp16.family}{0.790}
\@namedef{N@sf3b_official.casp16.len100-300}{0.711}
\@namedef{N@sf3b_official.casp16.len300-600}{0.760}
\@namedef{N@sf3b_official.casp16.len<100}{0.590}
\@namedef{N@sf3b_official.casp16.len>600}{0.547}
\@namedef{N@sf3b_official.casp16.no_family}{0.600}
\@namedef{N@sf3b_official.casp16.overall}{0.704}
\@namedef{N@sf3b_official.casp16.subset}{0.693}
\@namedef{N@sf3b_official.foldbench334.family}{0.884}
\@namedef{N@sf3b_official.foldbench334.len100-300}{0.823}
\@namedef{N@sf3b_official.foldbench334.len300-600}{0.914}
\@namedef{N@sf3b_official.foldbench334.len<100}{0.756}
\@namedef{N@sf3b_official.foldbench334.len>600}{0.821}
\@namedef{N@sf3b_official.foldbench334.no_family}{0.774}
\@namedef{N@sf3b_official.foldbench334.overall}{0.842}
\@namedef{N@sf3b_official.foldbench334.subset}{0.801}
\@namedef{N@truth.cameo2025.family}{1.000}
\@namedef{N@truth.cameo2025.len100-300}{1.000}
\@namedef{N@truth.cameo2025.len300-600}{1.000}
\@namedef{N@truth.cameo2025.len<100}{1.000}
\@namedef{N@truth.cameo2025.len>600}{1.000}
\@namedef{N@truth.cameo2025.no_family}{1.000}
\@namedef{N@truth.cameo2025.overall}{1.000}
\@namedef{N@truth.casp16.family}{1.000}
\@namedef{N@truth.casp16.len100-300}{1.000}
\@namedef{N@truth.casp16.len300-600}{1.000}
\@namedef{N@truth.casp16.len<100}{1.000}
\@namedef{N@truth.casp16.len>600}{1.000}
\@namedef{N@truth.casp16.no_family}{1.000}
\@namedef{N@truth.casp16.overall}{1.000}
\@namedef{N@truth.foldbench334.family}{1.000}
\@namedef{N@truth.foldbench334.len100-300}{1.000}
\@namedef{N@truth.foldbench334.len300-600}{1.000}
\@namedef{N@truth.foldbench334.len<100}{1.000}
\@namedef{N@truth.foldbench334.len>600}{1.000}
\@namedef{N@truth.foldbench334.no_family}{1.000}
\@namedef{N@truth.foldbench334.overall}{1.000}
\makeatother

